X-ray high-resolution spectroscopy reveals feedback in a Seyfert galaxy from an ultra fast wind with complex ionization and velocity structure

Winds outflowing from Active Galactic Nuclei (AGNs) may carry significant amount of mass and energy out to their host galaxies. In this paper we report the detection of a sub-relativistic outflow observed in the Narrow Line Seyfert 1 Galaxy IRAS17020+4544 as a series of absorption lines corresponding to at least 5 absorption components with an unprecedented wide range of associated column densities and ionization levels and velocities in the range of 23,000-33,000 km/s, detected at X-ray high spectral resolution (E/Delta E ~1000) with the ESA's observatory XMM-Newton. The charge states of the material constituting the wind clearly indicate a range of low to moderate ionization states in the outflowing gas and column densities significantly lower than observed in highly ionized ultra fast outflows. We estimate that at least one of the outflow components may carry sufficient energy to substantially suppress star formation, and heat the gas in the host galaxy. IRAS17020+4544 provides therefore an interesting example of feedback by a moderately luminous AGN hosted in a spiral galaxy, a case barely envisaged in most evolution models, which often predict that feedback processes take place in massive elliptical galaxies hosting luminous quasars in a post merger phase.

==> defs.tex <==
% Journal Definitions
\def\aa{AA}
\def\aap{AA}
\def\aj{AJ}
\def\apj{ApJ}
\def\apjl{ApJ}
\def\apjs{ApJS}
\def\mnras{MNRAS}
\def\araa{ARA\&A}
\def\nat{Nature}
%
% Common units
%
\def\arcsec{\ifmmode {''} \else ${''}$\fi}
\def\arcmin{\ifmmode {'} \else ${'}$\fi}
\def\deg{\ifmmode {^\circ} \else ${^\circ}$\fi}
\def\cc{\ifmmode {\rm cm}^{-3} \else cm$^{-3}$\fi}
\def\cl{\ifmmode {\rm cm}^{-2} \else cm$^{-2}$\fi}
\def\pcm2{\ifmmode {\rm cm}^{-2} \else cm$^{-2}$\fi}
\def\micron{\ifmmode \mu{\rm m} \else $\mu$m\fi}
\def\kms{\ifmmode {\rm km\,s}^{-1} \else km\,s$^{-1}$\fi}
\def\kmps{\ifmmode {\rm km\,s}^{-1} \else km\,s$^{-1}$\fi}
\def\Hubble{\ifmmode {\rm km\,s}^{-1}\,{\rm Mpc}^{-1}
        \else km\,s$^{-1}$\,Mpc$^{-1}$\fi}
\def\ergsec{\ifmmode {\rm ergs\;s}^{-1} \else ergs s$^{-1}$\fi}
\def\ergcms{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\fi}
\def\ergcmsA{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-1}\,{\rm \AA}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\,\AA$^{-1}$\fi}
\def\ergcmsHz{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-2}\,{\rm Hz}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\,Hz$^{-1}$\fi}
%
% Solar units
%
\def\Msun{\ifmmode M_{\odot} \else $M_{\odot}$\fi}
\def\Lsun{\ifmmode L_{\odot} \else $L_{\odot}$\fi}
%
% Cosmological parameters
%
\def\qo{\ifmmode q_{0} \else $q_{0}$\fi}
\def\Ho{\ifmmode H_{0} \else $H_{0}$\fi}
%
% Approximately less than and greater than signs
%
\def\ltsim{\raisebox{-.5ex}{$\;\stackrel{<}{\sim}\;$}}
\def\gtsim{\raisebox{-.5ex}{$\;\stackrel{>}{\sim}\;$}}
%
% Line designations
%
\def\ion#1#2{#1$\;${\small\rm\@Roman{#2}}\relax}
\def\hi{H {\sc i}}
\def\Halpha{H$\alpha$}
\def\Hbeta{H$\beta$}
\def\Hgamma{H$\gamma$}
\def\Hdelta{H$\delta$}
\def\lya{Ly$\alpha$}
\def\lyb{Ly$\beta$}
\def\lyg{Ly$\gamma$}
\def\hei{He\,{\sc i}}
\def\cii{C\,{\sc ii}}
\def\ciii{C\,{\sc iii}}
\def\civ{C\,{\sc iv}}
\newcommand {\lm}{$\lambda$}
\newcommand {\etal}{et al.}
\newcommand {\hut}{{HUT}}
\newcommand{\oi}{O~{\sc i}}
\newcommand{\ovi}{O~{\sc vi}}
\newcommand{\ovii}{O~{\sc vii}}
\newcommand{\oviii}{O~{\sc viii}}
\newcommand{\heii}{He~{\sc ii}}
\newcommand{\feii}{Fe~{\sc ii}}
\def\oiii{{[O\,{\sc iii}]}}
\def\nv{N~{\sc v}}
\def\niii{N~{\sc iii}}
\def\siiv{Si~{\sc iv}}
\def\siiii{Si~{\sc iii}}
\def\siii{Si~{\sc ii}}
\def\fei{Fe\,{\sc i}}
\def\feii{Fe\,{\sc ii}}
\def\feiii{Fe\,{\sc iii}}
\def\feiv{Fe\,{\sc iv}}
\def\fexx{Fe\,{\sc xx}}
\def\hi{H\,{\sc i}}
\def\hii{H\,{\sc ii}}
\def\hei{He\,{\sc i}}
\def\heii{He\,{\sc ii}}
\def\ci{C\,{\sc i}}
\def\cii{C\,{\sc ii}}
\def\ciii{\ifmmode {\rm C}\,{\sc iii} \else C\,{\sc iii}\fi}
\def\civ{\ifmmode {\rm C}\,{\sc iv} \else C\,{\sc iv}\fi}
\def\cv{\ifmmode {\rm C}\,{\sc v} \else C\,{\sc v}\fi}
\def\cvi{\ifmmode {\rm C}\,{\sc vi} \else C\,{\sc vi}\fi}
\def\ni{N\,{\sc i}}
\def\nii{N\,{\sc ii}}
\def\niii{N\,{\sc iii}}
\def\niv{N\,{\sc iv}}
\def\nv{N\,{\sc v}}
\def\nvi{N\,{\sc vi}}
\def\nvii{N\,{\sc vii}}
\def\oi{O\,{\sc i}}
\def\oii{O\,{\sc ii}}
\def\oiii{O\,{\sc iii}}
\def\o5007{[O\,{\sc iii}]\,$\lambda5007$}
\def\oiv{O\,{\sc iv}}
\def\ov{O\,{\sc v}}
\def\ovi{O\,{\sc vi}}
\def\ovii{O\,{\sc vii}}
\def\oviii{O\,{\sc viii}}
\def\neiii{Ne\,{\sc iii}}
\def\nev{Ne\,{\sc v}}
\def\neviii{Ne\,{\sc viii}}
\def\neix{Ne\,{\sc ix}}
\def\nex{Ne\,{\sc x}}
\def\mgi{Mg\,{\sc i}}
\def\mnii{Mn\,{\sc ii}}
\def\Niii{Ni\,{\sc ii}}
\def\mgii{Mg\,{\sc ii}}
\def\mgix{Mg\,{\sc ix}}
\def\mgx{Mg\,{\sc x}}
\def\mgxi{Mg\,{\sc xi}}
\def\siiv{Si\,{\sc iv}}
\def\siIII{Si\,{\sc iii}}
\def\siII{Si\,{\sc ii}}
\def\six{Si\,{\sc x}}
\def\sixi{Si\,{\sc xi}}
\def\sixii{Si\,{\sc xii}}
\def\sixiii{Si\,{\sc xiii}}
\def\si{S\,{\sc i}}
\def\sii{S\,{\sc ii}}
\def\siii{S\,{\sc iii}}
\def\siv{S\,{\sc iv}}
\def\sv{S\,{\sc v}}
\def\svi{S\,{\sc vi}}
\def\sx{S\,{\sc x}}
\def\sxi{S\,{\sc xi}}
\def\sxii{S\,{\sc xii}}
\def\sxiii{S\,{\sc xiii}}
\def\ariii{Ar\,{\sc iii}}
\def\ariv{Ar\,{\sc iv}}
\def\arv{Ar\,{\sc v}}
\def\arvi{Ar\,{\sc vi}}
\def\arvii{Ar\,{\sc vii}}
\def\arviii{Ar\,{\sc viii}}
\def\caii{Ca\,{\sc ii}}
\def\fei{Fe\,{\sc i}}
\def\feii{Fe\,{\sc ii}}
\def\feiii{Fe\,{\sc iii}}
\def\feix{Fe\,{\sc ix}}
\def\fexvii{Fe\,{\sc xvii}}
\def\fexviii{Fe\,{\sc xviii}}
\def\fexix{Fe\,{\sc xix}}
\def\fexxiii{Fe\,{\sc xxiii}}
\def\fexxiv{Fe\,{\sc xxiv}}
\def\fexxv{Fe\,{\sc xxv}}
\def\fexxvi{Fe\,{\sc xxvi}}
\def\alii{Al\,{\sc ii}}
\def\aliii{Al\,{\sc iii}}
\def\piv{P\,{\sc iv}}
\def\cliv{Cl\,{\sc iv}}
\def\clv{Cl\,{\sc v}}
\def\nai{Na\,{\sc i}}
%
\def\fek{{\rm Fe\,K$\alpha$}}
\def\fekb{{\rm Fe\,K$\beta$}}
\def\xmm{XMM-{\it Newton}}
\def\chandra{{\it Chandra}}

